Sending Money Like Sending E-mails: Cryptoaddresses, The Universal Decentralised Identities

Sending money in cryptocurrencies is majorly based on public keys or their hashed forms -- "addresses." These long random-looking strings are user unfriendly for transferring by other means than via copy-and-paste or QR codes. Replacing such strings with identifiers chosen by users themselves would significantly improve usability of cryptocurrencies. Such identifiers could be memorable, easier to write on paper or to dictate over phone. Main challenge lies in designing a practically usable decentralised system for providing these identifiers. Former solutions have been built as centralised systems or come with nonnegligible limitations. Our solution is reminiscent of a prevalent e-mail system, which is an already user friendly and desirably decentralised system. It is shown that our approach is directly applicable also to other systems that use long cryptographic identifiers.

==> eptcsdata.tex <==
\providecommand{\firstpage}{52}
\providecommand{\publicationstatus}{J. Bouda et al. (Eds.): 11th Doctoral Workshop\\
on  Mathematical and Engineering Methods\\
in Computer Science (MEMICS 2016)\\
EPTCS 233, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.233.5}{10.4204/EPTCS.233.5}}

